Smart Sports Predictions via Hybrid Simulation: NBA Case Study

Increased data availability has stimulated the interest in studying sports prediction problems via analytical approaches; in particular, with machine learning and simulation. We characterize several models that have been proposed in the literature, all of which suffer from the same drawback: they cannot incorporate rational decision-making and strategies from teams/players effectively. We tackle this issue by proposing hybrid simulation logic that incorporates teams as agents, generalizing the models/methodologies that have been proposed in the past. We perform a case study on the NBA with two goals: i) study the quality of predictions when using only one predictive variable, and ii) study how much historical data should be kept to maximize prediction accuracy. Results indicate that there is an optimal range of data quantity and that studying what data and variables to include is of extreme importance.

==> summary_lit_papers.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% SUMMARY IDEAS AND READING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Some possible ideas for the name of the paper are so far
\begin{enumerate}
    \item Smart sports predictions via hybrid simulation: NBA case study
    \item Smart sports predictions and decision-making via hybrid simulation: NBA case study
    \item Hybrid simulation for sports prediction: NBA Case study
    \item Hybrid simulation for sports prediction: evaluating the value of single summary statistics for the NBA.
    \item Creating and evaluating the value of statistics and statistical models under the presence of partial and uncomplete data via simulation: NBA case study
    \item Hybrid Simulation to construct accurate analytics and randomness models under noisy and partial data: NBA study case
    \item Hybrid simulation model to assess the value of analytics based on partial and noisy data: NBA case study
\end{enumerate}


\section{Introduction}

Some ideas for introduction and motivation:
\begin{itemize}
    

    
    \item Tradeoff on weighting more recent data: may be more indicative of present state of a team, but may also overfit to just current state of a team in particular! \textcolor{red}{I think I got the idea with the paper. How many ``last'' games to keep as a win percentage statistic gives a nice result?}

    \item Our approach is hybrid, since we consider games as events, but also teams are modeled as entities, and they may be given agent attributes. Future work: they could decide to rest players and so on. Carrying on their data allows this flexibility. Example of why it may be needed to include rational thinking? Injury prevention, ``big'' games with implications coming on, playoff seed already clinched (or already out of the race), among others.

    \item In our work we focus on simple models, easy to interpret. There is a trade-off in accuracy, but appeal is their wide usability, opportunity to generalize under more conditions, and also the fact that they are more valuable as information to be distributed for public.

    \item in our work we do not have controllable variables, but just a way to control what stochastic model is chosen, and what are the inputs for the model. We are essentially not trying to optimize the system, but trying to optimize the model and its parameters given on the real data such as to get an accurate description of the system.

    \item characteristics of our data? Incomplete (status for players?), partial (think just a couple of games), correlated (previous games played and so on), biased because each sample is taken under multiple different conditions.
\end{itemize}

Some notes taken from papers read so far:
\begin{itemize}
    \item from \shortcite{Nelson2016} ``simulation users are increasingly interested in utilizing stochastic simulation for risk analysis, prediction and control.'' Our model allows that by putting a stochastic modeling layer that takes data, produces win probabilities. Basically we allow for prediction and control over outcomes by simulating different randomness models?

    \item Also from \shortcite{Nelson2016}, simulation analytics. Embedding the model allows to compute and store the complete sample paths, and to understand the interaction of using partial data versus end of year data to check partial deviations. Basically, we can study the seasons as they move, not only at the end. -> May not be really applicable to what we do, so may need to revisit that section (number 4) later.
    

    \item On \shortcite{Ouyang2017}, the store and use the complete sample paths generated via simulation, instead of just some summary statistics. Their paper is basically a proof-of-concept and first step towards the use of predictive analytics that are derived from data obtained in the simulations. \note{This bodes well for our future work, where we can incorporate sample path data to understand better outcomes for teams. Particularly relevant since team data/sample paths for teams are very scarce. Just 30 per year!}


    \item \shortcite{Bowman2017} focus on what they refer to as ``retroactive gambling line simulation'' using NBA data. They basically use gambling lines such as to approximate winning probabilities for teams in any particular game, and based on that, they compare how impressive some accomplishments are, such as getting a large amount of wins, over the years. The need of having to approximate win probabilities for games comes from a three-sided perspective: i) Within years the quality of teams to be faced changes considerably, and so that affects how impressive may be to get an extreme amount of wins or not. ii) Even within the same year, teams face opponents a different amount of times, which makes impossible to give a fair comparison to seasons, unless accounting for the different in the ``strength'' of the opponents faced. iii) There exist different conditions that may affect runs of wins for teams, for instance facing teams with their best players injured increases the probability of winning, and so that needs to be accounted for when evaluating what season is more impressive. They use gambling lines as a proxy for win probabilities because they usually incorporate a lot of information that cannot be found in traditional statistics, such as last-minute injuries, suspensions, previous matchups, even particular referees on-court. Their approach is very different than most literature because they use the money spread instead of other estimators. Their methodology essentially uses these win probabilities to simulate the seasons many times and evaluate the probabilities of the outcomes, this is essentially seeing the season outcomes as one possible sample path for the season. 

    \item We have a tradeoff: more modeling complexity (say neural net or linear regression or whatever) versus simpler model (think binomial, bernoulli, etc).

    \item We are optimizing over a set of models, so we basically are optimizing how close our simulation model behaves compared to the sample paths observed (seasons)

    \note{Our model allows injection of more data, no assumptions as well!}

    \item \note{IN LIT REVIEW THERE MUST BE A DISTINCTION IN PAPERS SIMULATING PLAYS (PLAY BY PLAY), JUST GAMES OUTCOMES OR OTHERS}


    

    \item Most is use of historical data, but how long is long enough? This is meant of indication of non-stationarity (improvement, decline) of players or teams. \note{Refine idea}

    
\end{itemize}

\review{
Already used
\begin{itemize}
    \item The Big Data revolution continues to increase the data availability and collection. Companies and organizations make use of it and have shifted towards data-driven decision making with the goal of increasing performance. Having said that, using the data available effectively is a large challenge. In particular, data may be uncomplete, part of a larger series, or lead to bad outcomes if not taking into account the possible future behavior of the system (think greedy assignment, when more orders are arriving). 
    
    \item One of the more notable difficulties in modeling is being able to reproduce the essential system behavior while obtaining accurate predictions while utilizing a model that is simple enough to run. The new data availability allows to incorporate more of that real-time information embedded in the simulation models, with the hope that it will increase the model's validity, or improve predictions, but how to leverage that information within the simulation remains a design problem, and depends on the problem being considered. 

    \item Simulation is a powerful tool to test decision-making, and to validate the model building as well, in particular when some sources of randomness cannot be taken into consideration.

    \item From \shortcite{Eunji2023}, there is some ``observable-data'', in their words: ``observable data, in this setting, are not aligned with the full state necessary in order to initialize a dynamic simulation of the container system.'' We also suffer from ``incomplete data'' think not having all matchups!

    \item From \shortcite{Fu2002} describes simulation-optimization as the field that looks for the ``best'' inputs for our decision variables of simulated systems, with best roughly being equivalent to optimizing of (or many) metrics of interest. In his paper, he describes the process as being a two-step procedure, when the first step focuses on generating candidate solutions, and the second on evaluating them. Obviously, knowledge on how to generate ``good'' candidate solutions speeds up the process, and that is why search-based approaches and metaheuristics focusing on regions of the feasible area that have good partial results are used, however at the expense of not guaranteeing as outcome the true optimal solution.
    
    We can think of simulation-optimization as finding the best inputs for our decision variables of simulated systems. From Fu[15], SO can be divided in two phases: the first corresponds to the generation of possible candidates for the problem and the second corresponds to the evaluation of the induced solutions via estimations obtained by the repeated simulations.

    \item According to Miranda et al. [16], although several heuristic and metaheuristic techniques have been developed for optimization in simulation  environments over the last years, this research feld is still little explored.
    Furthermore, although SO is a powerful and flexible technique, it is important to note that, considering complex systems in which the search space for possible solutions is too large, its use may demand a long computational time to converge, making this approach infeasible. 

    \item In discrete event simulation (DES) models, stochastic behaviour is modelled by sampling random variates from probability distributions to determine event outcomes. However, the distribution of outcomes for an event from a real system is often dynamic and dependent on the current system state. This paper proposes the use of artificial neural networks (ANN) in DES models to determine the current distribution of each event outcome, conditional on the current model state or input data, from which random variates can then be sampled. This enables more realistic and accurate modelling of stochastic behaviour. An application is in digital twin models that aim to closely mimic a real system by learning from its past behaviour and utilising current data to predict its future. \shortcite{Reed2022} \note{Use this paper for introduction. We aim to model stochastic behavior with as little data as possible}

    \item \shortcite{Delafuente2018} demonstrate the feasibility of enabling smart processes in discrete event simulation software and the improved decision-making that may be induced by data-driven steps within the simulation. Main objective = how to build a smarter simulation model, integrating ML algorithms within the simulation.
    \item Also from \shortcite{Delafuente2018}, applications of ML on simulation can be divided in three main areas: ``Over the past two decades researchers have sought to incorporate machine learning into simulation to improve speed of execution, increase estimation accuracy, and reliable behavior. It is possible to categorize many of these simulation applications as being related to: 1) metamodeling and analysis, 2) parameter prediction, and 3) intelligent decision making.'' We may introduce ML as part of our prediction step, with the goal of improving estimation accuracy.

    \item \shortcite{Koning2001}``A simulation model for football championships''. Authors recognize a challenge similar to what we have initially: missing data to assess the strength level of a team. They also state that even if they knew the strength level of teams, they would need a stochastic model that returns winning probabilities for matches (or just the tournament). They use a two-step method: compute first a statistic that is meant to approximate the expected number of goals of a team A versus a team B, then use all of those expected values as input to a simulation model that returns the probability of being the champion. They assume the number of goals scored to be a poisson distribution for each team, and fit different estimators for matches based on historical data. Their approach differs from us as they assume a model and estimate strength of teams based on it, then compute probabilities based on it. Their analysis also allowed them to evaluate ``lucky draws'' based on the change of winning probabilities of a team when switching to a full-draw tournament. It allows for theoretical probability computations and all !

    \item \shortcite{Garnica2022} present what they describe as a simulation framework to analyse predictive models in sports, and claim using it may help to provide a better understanding on rating procedures and forecasting techniques for accurate predictions.

    \item he efficient market hypothesis posits that prices always reflect all available information, and loosely-based on that hypothesis, it is theorized that betting odds offer a type of predictor and source of expert advice regarding sports outcomes, and they have empirically performed well \shortcite{Spann2009}. In fact also shown that it is hard to beat betting even with state of the art models as seen in \shortcite{Manner2016} where they build upon linear model for team strengths, allowing for time-varying, but showing that strengths do not change too much over time; which they solve with ordinary least squares. Effects of back to backs and home advantage here are assumed to be EQUAL but that is not the case most of the time (i.e. NYK bad home advantage, OKC good,...) They also have normality assumption! From them: ``The effect of home advantage more or less + 2.7 points, the effect of back to backs more or less - 1.8; robust among different models and seasons. They found difficult to find differences in strength over the course of a season, and speculated that it was due to lack of enough data (since only 82 x 15 games). Percentage correct winner between 68 and 69 \% seasons 2006 to 2014, only using the second half of the season data as testing (so their parameters were tuned using the first half of the season, then recalibrated after each game), they also test for playoffs using regular season data to parameter computation, and obtain same accuracy.

    \item With respect to the effect of home advantage \shortcite{Ribeiro2016} also studied it from a team-varying and time dependent perspective, showing that the effect is different in both dimensions.

    \shortcite{Song2020} They model scores and predict win probabilities based on a Bivariate normal model depending on 5 performance statistics, including the four most important factors as studied in \shortcite{Kubatko2007}, parameters fitted with respect historical data. They also adjust the performance statistics with home and away splits and to the opposing team. Winning probas based on normality assumptions. LIT REVIEW!!
    They exhibit forecasting accuracies between 61\% and 68\%

     \item A common finding of many studies 
    is that predictions based on betting markets are difficult to beat, thus implying efficiency of the betting markets; see also Steckler et  al. (2010)

    \item Studying factors affecting quality of plays and in specific of shots \shortcite{Rolland2020}

    \item Recently deep learning methods have been used \shortcite{Yanai2022}, but with heavy reliance in data, and poor results on win estimation probabilities, very likely to the fact that the state space is too large for the amount of data available.


    \item It is a known fact that home teams perform better and visitants and there has been many aspects theorizing why. Refereeing biases have been shown to help to be in favor of the home team \cite{Pelechrinis2023}, and that is why it makes sense to use home/away splits

    \item One of the problems studied in sports is the prediction of outcomes of plays. In particular, \shortcite{Cervone2016} propose the use of optical player tracking data to estimate, in real time, what they define as expected possession value (EPV) for the NBA. Further studies have been done on studying the outcomes of multiple nba possessions over time, such as \shortcite{Sandholtz2018,Sandholtz2020} did by using Markov Decision Processes, and testing via simulation the outcome of changing policies (shooting distributions). \shortcite{Oh2015} uses a graphical model to treat the progression of a match as a graph, and simulate games (and their outcomes) based on different lineups as input, which can be used for decision support. Their process is data-driven but all the distributions set in advance for different outcomes of possessions, and determined from the lineups data, which means it cannot generalize to players on new teams for example.

    \shortcite{Vracar2016} is a simulation of basketball games as a sequence of play-by-play situations from teams, also using MDP, but adding time and score difference to the state space such as to provide for a better representation of reality. They use 8 summary statistics as a proxy for team characteristics. They do home and away split of stats, and even though they conclude their results generalize well for play-to-play transitions, they systematically overrate bad teams and underrate good teams with their projected wins based on the model.

    \item Note that the play-by-play methods have many uses but they are not suitable to explain differences in schedule strength or stuff like that, since they are data-tailored to the teams and specific lineups, and so any changes made to schedules to evaluate their difficulty would introduce other biases such as team composition and so on, but also that the models themselves may be trained on the head-to-head data, so they are not to be used to measure what a "neutral" or "hard" schedule is.

    While interesting, non-linearity of policies makes models limited to their neighborhoods (for example, increasing shooting of threes may just reduce their quality and percentage, but that interaction in unknown). 

    Also the need for simple indicators of how a team is. One of the first ideas to estimate the number of wins is the Pythagorean expectation from Bill James, devised initially for baseball but then adapted for multiple sports\footnote{\url{https://en.wikipedia.org/wiki/Pythagorean_expectation}}, which basically returns a number of expected wins given a two statistics that may be representative of team strength in offense and defense. Simple, uncorrelated, nice approximation of wins, but what about their predictive power?
    
\end{itemize}


}











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% PREVIOUS METHODOLOGY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
So far in Section \ref{sec:lit_review} we presented many influential works where the goal is to predict the outcome of a sports game/match. Even though many of those models are used for different sports, are based on different methods and come from different areas of knowledge, they can be divided in four large common categories: 1) stochastic simulation models, 2) play-by-play simulation models, 3) ML-based models and a 4) tournament model. We will explain how all of them can actually be seen as a special kind of discrete-event simulation model:
\begin{enumerate}
    \item [1)]With respect to i), each game is an event and the outcomes are computed based on statistical distributions, and random values sampled from them. The statistical distributions are based out of expert knowledge and past data, just as the distribution parameters.  
    \item [2)] Play-by-play simulation models are usually based on Markov Chains or an extension such as Markov Decision Processes. Here events are basically plays, and the next state (play) just depends on the previous. Granularity of the model may vary, but it is clear how this is a discrete event model, even if a sequence of games is simulated, in which case we would have two types of events, and the play-by-play framework would lie within a i) type model.
    \item [3)] With respect to ML-based methods, we note the following: the construction of the datasets requires the design choice of how much and what data to include, but also what is the desired ``event'' unit, which most of the time is a game/match. Then, based on that, a ML algorithm is trained on a training set, and the resulting model is used for prediction. This is a discrete-event model because over the test scenario, each game can be seen as an ``independent'' event, where the outcome will be obtained after using the ML model (and maybe sampling for a random uniform). In reality the events/test samples are not ``independent'' since most of the time the dataset will contain information from the real games played recently, so observations are correlated, however within the ML test set, we can see each sample as an ``independent'' event that is not influenced by the outcome of the prediction from previous samples.
    \item [4)] Tournament models are discrete event models because each game corresponds to an event, and the tournament is just an ordered sequence of games, where the outcome of previous games may (example: soccer world cup), or may not (i.e. soccer league) determine the following matchups, and previous games may (or not) even the winning probabilities. Note that here the simulation of each game may be done with any of the models i), ii) or iii); and the tournament may (or not) follow a Markovian property.
\end{enumerate}

Some of the models may be considered hybrid because of including several methods/algorithms within the simulation, however they all suffer from a large drawback: they cannot incorporate ``result-strategy''/game-theory within the model, unless it is at the expense of an extremely large increase in the complexity of their state space. Some examples that highlight why incorporating team/player logic and agent-based behavior may be relevant are:
\begin{itemize}
    \item \href{https://www.uefa.com/uefachampionsleague/}{The UEFA Champions League} is the most important soccer club competition in the world, and features many double-game elimination matchups (with one ``away'' and one ``home'' game), and it is widely known how a positive or negative result on the first match affects the strategy of the team in the second game, as they can go to the next round with a draw or a loss with small difference. This same tournament also features a \href{https://en.wikipedia.org/wiki/Round-robin_tournament}{double round-robin style} group stage, where groups of four teams compete for two positions on the next round. Under some conditions, one of the teams may be already eliminated when playing a game, in which case they may not feature their starter team. In others, two teams may guarantee passing to the next round with a draw, whereas a loss may mean not passing; in which case a draw is a ``good'' result for both teams, and affects how the match is played from a strategy standpoint. 
    \item On tennis tournaments, it is common for less-known players to play both the singles and doubles version. On some opportunities some players advance to final rounds in both, and thus some strategy kicks-in. Load manage or even retire from one of the tournaments to increase chances in the other? Play both at best effort, which likely means the second match of the day will have an unrested player? This should be a part of the strategy for maximum accuracy of forecasting purposes.
    \item On tournaments with unequal rest between matches, there is frequent load managing. This happens with soccer cups that are played mid-week (think FA cup in England), in particular if the opponent is from a lower league. Another good example is the NBA, where many star players rest one game if there is two on consecutive days. Under that scenario, what game does player play-in? Most of the time that is decided by the team with some goal in mind, usually increasing their win expectations.
\end{itemize}

Hopefully, the past examples explain \textbf{why} there is a need to somehow include ``look-ahead'' strategy from teams/players. Now, while that can be done by expanding the state space on previous models, that may not be possible for models of type ii), and that may just increase significantly the state space of models of type i) and iii) by adding more discrete variables, usually binary variables that indicate some condition on the match that may induce some different strategy; and that also may come at the heavy price of over fitting if that is not a common condition. 

Having said that, we propose a hybrid simulation model that incorporates agent-based logic such as to tackle this issue without adding too much extra complexity, also allowing to test the performance of different strategies, and to consider agents that may react differently under the same conditions because of some of their attributes. Our modeling approach works at a game prediction level however the same ideas could be adapted into a game-to-game concept. In particular, the model considers up to four different levels of granularity, each represented by a class, and each instance of a class having some particular attributes; as seen in figure.....

\begin{figure}[h!]
    \centering
    \includegraphics[scale=.77]{Figures/QueueSimNotepad.pdf}
    \caption{Offering procedure.}
    \label{Fig:StructureClasses}
\end{figure}{}

\fi




%%%%%%%%%%%%%%%%%%%%%%%%% FIGURES

\iffalse
\begin{figure}
\begin{center}
\begin{subfigure}{.49\textwidth}
  \centering
  % include first image
  \includegraphics[width=0.99\linewidth]{WSC2023_LatexTemplates/Figures/2021-2022_online_largest_val_netrat_all.pdf}  
  \caption{Offline Bernoulli Race --- Method (i)}
  \label{fig:OfflineBernoulli}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  % include second image
  \includegraphics[width=0.99\linewidth]{Figures/2021-2022_online_bernoulli_all.pdf}  
  \caption{Online Bernoulli Race --- Method (ii)}
  \label{fig:OnlineBernoulli}
\end{subfigure}
\caption{Results of the test set for the liver model.}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\begin{subfigure}{.49\textwidth}
  \centering
  % include first image
  \includegraphics[width=0.99\linewidth]{WSC2023_LatexTemplates/Figures/bernoulli_lags_home_2021-2022.pdf}  
  \caption{Offline Bernoulli Race --- Method (i)}
  \label{fig:LagsBenoulliHome}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  % include second image
  \includegraphics[width=0.99\linewidth]{WSC2023_LatexTemplates/Figures/bernoulli_lags_home_sec_half_2021-2022.pdf}  
  \caption{Online Bernoulli Race --- Method (ii)}
  \label{fig:LagsBernoulliHomeSecondHalf}
\end{subfigure}
\caption{Results of the test set for the liver model.}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\begin{subfigure}{.49\textwidth}
  \centering
  % include first image
  \includegraphics[width=\textwidth]{Figures/2021-2022_retrospective_bernoulli_all.pdf}  
  \caption{Offline Bernoulli Race --- Method (i)}
  \label{fig:OfflineBernoulli}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{Figures/2021-2022_online_bernoulli_all.pdf}  
  \caption{Online Bernoulli Race --- Method (ii)}
  \label{fig:OnlineBernoulli}
\end{subfigure}
\caption{Results of the test set for the liver model.}
\end{center}
\end{figure}

\fi


%%%%%%%%%%%%%%%%%%%%%% OLD INTRODUCTION

\section{Introduction}
Over the last decades, the Big Data revolution has increased data collection, availability and usage. Companies and organizations have shifted towards data-driven decision making such as to improve performance; however making good use of the data is still a large challenge. Under this context, simulation is used as a powerful tool that allows to evaluate the value, contribution and best setup for the data that is available, and also to optimize the performance of the system being considered. Furthermore, one of the hardest steps when building a simulation model is being able to reproduce the most notable aspects of the system, all while being a fast model that allows to obtain the desired statistics and optimize the metrics of interest; and that is why there also exists synergy with the new data availability, as the data can be used to build more reliable and robust simulation models. In the past, discrete-event simulation, system dynamics and agent-based simulation were the main paradigms but lately new paradigms better suited to incorporate intelligent frameworks that leverage data (such as machine learning) are gaining steam; in particular hybrid models and metamodels.

Prediction is a relevant problem in most areas of study, and while the big era data has facilitated its study through Machine Learning lens, there are problems where conventional algorithms are not enough and more sophisticated approaches need to be considered. In the recent paper ``Simulation-based Prediction'' \shortcite{Eunji2023} argue towards the use of simulation as they work with a complicated system where there is some ``observable-data'' that is not necessarily aligned with the full state/data of the system, and so simulation ends up being a necessary tool to improve their decisions/predictions. In particular, sports prediction is a really hard problem because: i) a very small amount of ``observable-data'' from games does not describe all the state of the system (health and quality of players, strategies of teams, interactions between players, \ldots), ii) correlated data (teams/players against each other), iii) time-varying data in a setting where the ``non-observable'' variables can change significantly, iv) a non-complete data space (all pairs of players may have not played each other yet). 

\note{IMPROVE THIS}Having said this we propose a hybrid simulation approach for sports prediction, and use as case study the NBA, where we show how powerful and flexible the modeling framework is by evaluating the value of single summary statistics for prediction purposes. The rest of the paper is as follows: in Section \ref{sec:lit_review} we present a literature review focused on sports and prediction, Section \ref{sec:methodology} explains our methodology, in Section \ref{sec:case_study} we introduce our case study, present our simulation results and discuss them, finally Section \ref{sec:conclusions} provides our conclusions. 

==> wsc23style.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% File contains:
%   fancyhdr.sty
%   psfig.sty
%   url.sty
%   wsc.bst
%   wscpaperproc.cls
%   wscsetup.sty
%   wsc.sty
%   wscbib.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



